A Markov Reward Process-Based Approach to Spatial Interpolation

The interpolation of spatial data can be of tremendous value in various applications, such as forecasting weather from only a few measurements of meteorological or remote sensing data. Existing methods for spatial interpolation, such as variants of kriging and spatial autoregressive models, tend to suffer from at least one of the following limitations: (a) the assumption of stationarity, (b) the assumption of isotropy, and (c) the trade-off between modelling local or global spatial interaction. Addressing these issues in this work, we propose the use of Markov reward processes (MRPs) as a spatial interpolation method, and we introduce three variants thereof: (i) a basic static discount MRP (SD-MRP), (ii) an accurate but mostly theoretical optimised MRP (O-MRP), and (iii) a transferable weight prediction MRP (WP-MRP). All variants of MRP interpolation operate locally, while also implicitly accounting for global spatial relationships in the entire system through recursion. Additionally, O-MRP and WP-MRP no longer assume stationarity and are robust to anisotropy. We evaluated our proposed methods by comparing the mean absolute errors of their interpolated grid cells to those of 7 common baselines, selected from models based on spatial autocorrelation, (spatial) regression, and deep learning. We performed detailed evaluations on two publicly available datasets (local GDP values, and COVID-19 patient trajectory data). The results from these experiments clearly show the competitive advantage of MRP interpolation, which achieved significantly lower errors than the existing methods in 23 out of 40 experimental conditions, or 35 out of 40 when including O-MRP.

==> Chapters/Tables/covid.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\resizebox{0.8\textwidth}{!}{%
\begin{tabular}{lllllllllllll}
\hline
\multicolumn{1}{c}{}                                    & \multicolumn{12}{c}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\
\multicolumn{1}{c}{\multirow{-2}{*}{}}                  & \multicolumn{12}{c}{\multirow{-2}{*}{\textbf{Test data:   Daegu (COVID-19)}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{6}{c|}{\textbf{Training data: Daegu}}                                                                                                                                                                                                                                                & \multicolumn{6}{c|}{\textbf{Training data: Seoul}}                                                                                                                                                                                                                                                \\ \cline{2-13} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{2}{c|}{p=0.1}                                                               & \multicolumn{2}{c|}{p=0.5}                                                              & \multicolumn{2}{c|}{p=0.9}                                                                                   & \multicolumn{2}{c|}{p=0.1}                                                              & \multicolumn{2}{c|}{p=0.5}                                                              & \multicolumn{2}{c|}{p=0.9}                                                                                    \\ \cline{2-13} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Method}}} & \multicolumn{1}{c}{$\mu$}                                & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                                & \multicolumn{1}{c|}{$\sigma$}                      \\ \hline
\multicolumn{1}{|l|}{OK}                                & \cellcolor[HTML]{F8CECC}12.365$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.342 & \cellcolor[HTML]{F8CECC}13.04$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.513 & \cellcolor[HTML]{F8CECC}13.4$^{(\otimes)}$              & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.202} & \cellcolor[HTML]{F8CECC}12.99$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.303 & \cellcolor[HTML]{F8CECC}12.99$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.495 & \cellcolor[HTML]{F8CECC}13.203$^{(\otimes)}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.399} \\
\multicolumn{1}{|l|}{UK}                                & \cellcolor[HTML]{F8CECC}12.546$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.511 & \cellcolor[HTML]{F8CECC}13.18$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.313 & \cellcolor[HTML]{F8CECC}13.48$^{(\otimes)}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.444} & \cellcolor[HTML]{F8CECC}12.7$^{(\otimes)}$              & \cellcolor[HTML]{F8CECC}1.681 & \cellcolor[HTML]{F8CECC}12.85$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.676 & \cellcolor[HTML]{F8CECC}13.14$^{(\otimes)}$              & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.56}  \\
\multicolumn{1}{|l|}{Basic}                             & 2.5754                                                   & 0.234                         & 2.175                                                   & 0.606                         & 1.837                                                   & \multicolumn{1}{l|}{1.625}                         & 5.888                                                   & 1.914                         & 6.939                                                   & 0.911                         & 7.1245                                                   & \multicolumn{1}{l|}{0.767}                         \\
\multicolumn{1}{|l|}{SAR}                               & \cellcolor[HTML]{D5E8D5}1.1801$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}0.836 & \cellcolor[HTML]{D5E8D5}1.63$^{\mathbf{(3)}}$           & \cellcolor[HTML]{D5E8D5}0.629 & 2.402                                                   & \multicolumn{1}{l|}{1.632}                         & 4.362                                                   & 3.4                           & 3.902                                                   & 2.124                         & 3.787                                                    & \multicolumn{1}{l|}{3.261}                         \\
\multicolumn{1}{|l|}{MA}                                & 1.7667                                                   & 0.395                         & 2.25                                                    & 7.824                         & 3.699$^{\otimes}$                                       & \multicolumn{1}{l|}{83}                            & 4.519                                                   & 2.465                         & 5.157                                                   & 2.952                         & 3.835                                                    & \multicolumn{1}{l|}{2.641}                         \\
\multicolumn{1}{|l|}{ARMA}                              & 2.0881                                                   & 1.26                          & 2.064                                                   & 0.675                         & 2.315                                                   & \multicolumn{1}{l|}{2.227}                         & 4.404                                                   & 1.941                         & 4.181                                                   & 1.725                         & 3.8086                                                   & \multicolumn{1}{l|}{1.777}                         \\
\multicolumn{1}{|l|}{CNN}                               & \cellcolor[HTML]{D5E8D5}1.7525$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.247 & 2.227                                                   & 0.662                         & \cellcolor[HTML]{D5E8D5}1.364$^{\mathbf{(2)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}1.97}  & \cellcolor[HTML]{D5E8D5}1.844$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.05  & \cellcolor[HTML]{D5E8D5}1.857$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.049 & 2.0935                                                   & \multicolumn{1}{l|}{0.076}                         \\ \hline
\multicolumn{1}{|l|}{SD-MRP}                            & 1.1273                                                   & 2.399                         & \cellcolor[HTML]{D5E8D5}1.41$^{\mathbf{(2)}}$           & \cellcolor[HTML]{D5E8D5}0.699 & \cellcolor[HTML]{D5E8D5}1.753$^{\mathbf{(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.248} & \cellcolor[HTML]{D5E8D5}1.204$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}1.745 & \cellcolor[HTML]{D5E8D5}1.895$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.467 & \cellcolor[HTML]{D5E8D5}1.7843$^{\mathbf{(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.125} \\
\multicolumn{1}{|l|}{WP-MRP}                            & 2.0035                                                   & 2.427                         & \cellcolor[HTML]{D5E8D5}1.632$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.679 & 1.67                                                    & \multicolumn{1}{l|}{0.245}                         & \cellcolor[HTML]{D5E8D5}2.056$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}2.958 & \cellcolor[HTML]{D5E8D5}3.962$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}15.4  & \cellcolor[HTML]{D5E8D5}1.6638$^{\mathbf{(2)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.221} \\ \hline
\multicolumn{1}{|l}{O-MRP}                              & \cellcolor[HTML]{D5E8D5}\textbf{0.2647$^{\mathbf{(1)}}$} & 0.311                         & \cellcolor[HTML]{D5E8D5}\textbf{0.757$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.366 & \cellcolor[HTML]{D5E8D5}\textbf{1.197$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.253                      & \cellcolor[HTML]{D5E8D5}\textbf{0.243$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.402 & \cellcolor[HTML]{D5E8D5}\textbf{1.091$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.448 & \cellcolor[HTML]{D5E8D5}\textbf{1.6416$^{\mathbf{(1)}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.152} \\ \hline
\end{tabular}%
}
\caption{Results for COVID-19 interpolation methods in terms of the MAE mean and standard deviation from 30 runs per condition. The first to third best performing methods have been marked with the superscript $\mu^{(1)}$, $\mu^{(2)}$ or $\mu^{(3)}$ and a green background, and the worst performing method has been marked with $\mu^{(\otimes)}$ and a red background. Rankings were determined using statistical significance testing at $\alpha=0.05$  (ties allowed). The lowest error per condition, regardless of statistical significance, was marked \textbf{bold}.}
\label{tab:covid}
\end{table*}






% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \centering
% \resizebox{0.65\textwidth}{!}{%
% \begin{tabular}{lllllllllllll}
% \hline
% \multicolumn{1}{c}{}                                    & \multicolumn{12}{c}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\
% \multicolumn{1}{c}{\multirow{-2}{*}{}}                  & \multicolumn{12}{c}{\multirow{-2}{*}{\textbf{Test data:   Daegu (COVID-19)}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \hline
% \multicolumn{1}{|c|}{}                                  & \multicolumn{6}{c|}{\textbf{Training data: Daegu}}                                                                                                                                                                                                                                          & \multicolumn{6}{c|}{\textbf{Training data: Seoul}}                                                                                                                                                                                                                                          \\ \cline{2-13} 
% \multicolumn{1}{|c|}{}                                  & \multicolumn{2}{c|}{p=0.1}                                                             & \multicolumn{2}{c|}{p=0.5}                                                            & \multicolumn{2}{c|}{p=0.9}                                                                                 & \multicolumn{2}{c|}{p=0.1}                                                            & \multicolumn{2}{c|}{p=0.5}                                                            & \multicolumn{2}{c|}{p=0.9}                                                                                  \\ \cline{2-13} 
% \multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Method}}} & \multicolumn{1}{c}{$\mu$}                              & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                              & \multicolumn{1}{c|}{$\sigma$}                      \\ \hline
% \multicolumn{1}{|l|}{OK}                                & \cellcolor[HTML]{F8CECC}12.365$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.342 & \cellcolor[HTML]{F8CECC}13.04$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.513 & \cellcolor[HTML]{F8CECC}13.4$^{\otimes}$              & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.202} & \cellcolor[HTML]{F8CECC}12.99$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.303 & \cellcolor[HTML]{F8CECC}12.99$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.495 & \cellcolor[HTML]{F8CECC}13.203$^{\otimes}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.399} \\
% \multicolumn{1}{|l|}{UK}                                & \cellcolor[HTML]{F8CECC}12.546$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.511 & \cellcolor[HTML]{F8CECC}13.18$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.313 & \cellcolor[HTML]{F8CECC}13.48$^{\otimes}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.444} & \cellcolor[HTML]{F8CECC}12.7$^{\otimes}$              & \cellcolor[HTML]{F8CECC}1.681 & \cellcolor[HTML]{F8CECC}12.85$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.676 & \cellcolor[HTML]{F8CECC}13.14$^{\otimes}$              & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.56}  \\
% \multicolumn{1}{|l|}{Basic}                             & 2.5754                                                 & 0.234                         & 2.175                                                 & 0.606                         & 1.837                                                 & \multicolumn{1}{l|}{1.625}                         & 5.888                                                 & 1.914                         & 6.939                                                 & 0.911                         & 7.1245                                                 & \multicolumn{1}{l|}{0.767}                         \\
% \multicolumn{1}{|l|}{SAR}                               & \cellcolor[HTML]{D5E8D5}1.1801$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}0.836 & \cellcolor[HTML]{D5E8D5}1.63$^{\mathbf{3}}$           & \cellcolor[HTML]{D5E8D5}0.629 & 2.402                                                 & \multicolumn{1}{l|}{1.632}                         & 4.362                                                 & 3.4                           & 3.902                                                 & 2.124                         & 3.787                                                  & \multicolumn{1}{l|}{3.261}                         \\
% \multicolumn{1}{|l|}{MA}                                & 1.7667                                                 & 0.395                         & 2.25                                                  & 7.824                         & 3.699$^{\otimes}$                                     & \multicolumn{1}{l|}{83}                            & 4.519                                                 & 2.465                         & 5.157                                                 & 2.952                         & 3.835                                                  & \multicolumn{1}{l|}{2.641}                         \\
% \multicolumn{1}{|l|}{ARMA}                              & 2.0881                                                 & 1.26                          & 2.064                                                 & 0.675                         & 2.315                                                 & \multicolumn{1}{l|}{2.227}                         & 4.404                                                 & 1.941                         & 4.181                                                 & 1.725                         & 3.8086                                                 & \multicolumn{1}{l|}{1.777}                         \\
% \multicolumn{1}{|l|}{CNN}                               & \cellcolor[HTML]{D5E8D5}1.7525$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.247 & 2.227                                                 & 0.662                         & \cellcolor[HTML]{D5E8D5}1.364$^{\mathbf{2}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}1.97}  & \cellcolor[HTML]{D5E8D5}1.844$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.05  & \cellcolor[HTML]{D5E8D5}1.857$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.049 & 2.0935                                                 & \multicolumn{1}{l|}{0.076}                         \\ \hline
% \multicolumn{1}{|l|}{SD-MRP}                            & 1.1273                                                 & 2.399                         & \cellcolor[HTML]{D5E8D5}1.41$^{\mathbf{2}}$           & \cellcolor[HTML]{D5E8D5}0.699 & \cellcolor[HTML]{D5E8D5}1.753$^{\mathbf{3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.248} & \cellcolor[HTML]{D5E8D5}1.204$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}1.745 & \cellcolor[HTML]{D5E8D5}1.895$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.467 & \cellcolor[HTML]{D5E8D5}1.7843$^{\mathbf{3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.125} \\
% \multicolumn{1}{|l|}{WP-MRP}                            & 2.0035                                                 & 2.427                         & \cellcolor[HTML]{D5E8D5}1.632$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.679 & 1.67                                                  & \multicolumn{1}{l|}{0.245}                         & \cellcolor[HTML]{D5E8D5}2.056$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}2.958 & \cellcolor[HTML]{D5E8D5}3.962$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}15.4  & \cellcolor[HTML]{D5E8D5}1.6638$^{\mathbf{2}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.221} \\ \hline
% \multicolumn{1}{|l}{O-MRP}                              & \cellcolor[HTML]{D5E8D5}\textbf{0.2647$^{\mathbf{1}}$} & 0.311                         & \cellcolor[HTML]{D5E8D5}\textbf{0.757$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.366 & \cellcolor[HTML]{D5E8D5}\textbf{1.197$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.253                      & \cellcolor[HTML]{D5E8D5}\textbf{0.243$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.402 & \cellcolor[HTML]{D5E8D5}\textbf{1.091$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.448 & \cellcolor[HTML]{D5E8D5}\textbf{1.6416$^{\mathbf{1}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.152} \\ \hline
% \end{tabular}%
% }
% \caption{Results for COVID-19 interpolation methods in terms of the MAE mean and standard deviation from 30 runs per condition. The first to third best performing methods have been marked with the superscript $\mu^{1}$, $\mu^{2}$ or $\mu^{3}$ and a green background, and the worst performing method has been marked with $\mu^{\otimes}$ and a red background. Rankings were determined using statistical significance testing at $\alpha=0.05$  (ties allowed). The lowest error per condition, regardless of statistical significance, was marked \textbf{bold}.}
% \label{tab:covid}
% \end{table*}


==> Chapters/Tables/gdp.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\resizebox{1.2\textwidth}{!}{%
\begin{tabular}{lllllllllllllllllll}
\hline
\multicolumn{1}{c}{}                                    & \multicolumn{18}{c}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\
\multicolumn{1}{c}{\multirow{-2}{*}{}}                  & \multicolumn{18}{c}{\multirow{-2}{*}{\textbf{Test data:   Taipei (GDP)}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{6}{c|}{\textbf{Training data: Taipei}}                                                                                                                                                                                                                                               & \multicolumn{6}{c|}{\textbf{Training data: Seoul}}                                                                                                                                                                                                                                                & \multicolumn{6}{c|}{\textbf{Training data: Taichung}}                                                                                                                                                                                                                                                 \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{2}{c|}{p=0.1}                                                               & \multicolumn{2}{c|}{p=0.5}                                                              & \multicolumn{2}{c|}{p=0.9}                                                                                   & \multicolumn{2}{c|}{p=0.1}                                                              & \multicolumn{2}{c|}{p=0.5}                                                              & \multicolumn{2}{c|}{p=0.9}                                                                                    & \multicolumn{2}{c|}{p=0.1}                                                               & \multicolumn{2}{c|}{p=0.5}                                                              & \multicolumn{2}{c|}{p=0.9}                                                                                       \\ \cline{2-19} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Method}}} & \multicolumn{1}{c}{$\mu$}                                & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                                & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                                & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                                   & \multicolumn{1}{c|}{$\sigma$}                      \\ \hline
\multicolumn{1}{|l|}{OK}                                & \cellcolor[HTML]{D5E8D5}2.6301$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.233 & \cellcolor[HTML]{D5E8D5}2.629$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.244 & \cellcolor[HTML]{D5E8D5}\textbf{2.615$^{\mathbf{(1)}}$} & \multicolumn{1}{l|}{0.232}                         & 10.11                                                   & 0.589                         & 10.15                                                   & 0.583                         & 9.8365                                                   & \multicolumn{1}{l|}{0.465}                         & \cellcolor[HTML]{D5E8D5}2.5661$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.276 & \cellcolor[HTML]{D5E8D5}\textbf{2.504$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.233 & \cellcolor[HTML]{D5E8D5}2.692$^{\mathbf{(1),(2)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.252} \\
\multicolumn{1}{|l|}{UK}                                & \cellcolor[HTML]{D5E8D5}2.6704$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.236 & \cellcolor[HTML]{D5E8D5}2.593$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.223 & \cellcolor[HTML]{D5E8D5}2.727$^{\mathbf{(2)}}$          & \multicolumn{1}{l|}{0.249}                         & 10.19                                                   & 0.835                         & 10.41                                                   & 0.659                         & 10.317                                                   & \multicolumn{1}{l|}{0.74}                          & \cellcolor[HTML]{D5E8D5}2.6261$^{\mathbf{(2),(3)}}$      & \cellcolor[HTML]{D5E8D5}0.24  & \cellcolor[HTML]{D5E8D5}2.601$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}0.382 & \cellcolor[HTML]{D5E8D5}\textbf{2.649$^{\mathbf{(1),(2)}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.223} \\
\multicolumn{1}{|l|}{Basic}                             & 3.9129                                                   & 0.108                         & 3.779                                                   & 0.355                         & 3.451                                                   & \multicolumn{1}{l|}{0.857}                         & \cellcolor[HTML]{F8CECC}26.68$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}4.757 & \cellcolor[HTML]{F8CECC}26.27$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.704 & \cellcolor[HTML]{F8CECC}26.483$^{(\otimes)}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}0.306} & 4.9292                                                   & 1.705                         & 5.225                                                   & 0.753                         & 5.069                                                       & \multicolumn{1}{l|}{0.24}                          \\
\multicolumn{1}{|l|}{SAR}                               & 3.5778                                                   & 0.532                         & 4.164                                                   & 0.488                         & \cellcolor[HTML]{F8CECC}5.709$^{(\otimes)}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.659} & 7.972                                                   & 1037                          & 8.681                                                   & 1.585                         & 8.6299                                                   & \multicolumn{1}{l|}{1.298}                         & 5.7945                                                   & 2.396                         & \cellcolor[HTML]{F8CECC}5.913$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}13.95 & \cellcolor[HTML]{F8CECC}6.018$^{(\otimes)}$                 & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}104.5} \\
\multicolumn{1}{|l|}{MA}                                & 3.664                                                    & 0.556                         & 3.745                                                   & 0.505                         & 4.204                                                   & \multicolumn{1}{l|}{1.827}                         & 9.064                                                   & 8.498                         & 8.413                                                   & 5.201                         & 9.0289                                                   & \multicolumn{1}{l|}{12.25}                         & \cellcolor[HTML]{F8CECC}6.4553$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}2277  & \cellcolor[HTML]{F8CECC}6.365$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}22.67 & 6.083                                                       & \multicolumn{1}{l|}{17.24}                         \\
\multicolumn{1}{|l|}{ARMA}                              & 3.9379                                                   & 0.569                         & 4.067                                                   & 0.728                         & 4.386                                                   & \multicolumn{1}{l|}{0.689}                         & 9.46                                                    & 5.503                         & 9.446                                                   & 7.303                         & 10.939                                                   & \multicolumn{1}{l|}{4.77}                          & 5.4766                                                   & 0.884                         & 5.443                                                   & 1.067                         & 6.15                                                        & \multicolumn{1}{l|}{1.072}                         \\
\multicolumn{1}{|l|}{CNN}                               & \cellcolor[HTML]{F8CECC}5.469$^{(\otimes)}$              & \cellcolor[HTML]{F8CECC}0.378 & \cellcolor[HTML]{F8CECC}5.481$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.811 & 4.79                                                    & \multicolumn{1}{l|}{2.259}                         & \cellcolor[HTML]{D5E8D5}5.676$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.242 & 5.606                                                   & 0.245                         & \cellcolor[HTML]{D5E8D5}5.7203$^{\mathbf{(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.238} & 5.5233                                                   & 2.251                         & 5.509                                                   & 1.454                         & 5.537                                                       & \multicolumn{1}{l|}{13.89}                         \\ \hline
\multicolumn{1}{|l|}{SD-MRP}                            & 3.7774                                                   & 1.981                         & 4.585                                                   & 0.736                         & 5.262                                                   & \multicolumn{1}{l|}{0.329}                         & \cellcolor[HTML]{D5E8D5}3.695$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}1.348 & \cellcolor[HTML]{D5E8D5}4.582$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}0.508 & \cellcolor[HTML]{D5E8D5}5.3042$^{\mathbf{(2)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.557} & 3.869                                                    & 1.451                         & 4.301                                                   & 0.409                         & \cellcolor[HTML]{D5E8D5}4.75$^{\mathbf{(3)}}$               & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.442} \\
\multicolumn{1}{|l|}{WP-MRP}                            & 4.9688                                                   & 2.243                         & \cellcolor[HTML]{F8CECC}5.382$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.723 & 5.296                                                   & \multicolumn{1}{l|}{0.263}                         & \cellcolor[HTML]{D5E8D5}6.089$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}2.464 & \cellcolor[HTML]{D5E8D5}5.322$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.781 & 5.2046                                                   & \multicolumn{1}{l|}{0.297}                         & 5.4675                                                   & 2.538                         & 5.284                                                   & 0.962                         & 5.183                                                       & \multicolumn{1}{l|}{0.319}                         \\ \hline
\multicolumn{1}{|l|}{O-MRP}                             & \cellcolor[HTML]{D5E8D5}\textbf{0.9534$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.514 & \cellcolor[HTML]{D5E8D5}\textbf{1.753$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.343 & \cellcolor[HTML]{D5E8D5}3.021$^{\mathbf{(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.746} & \cellcolor[HTML]{D5E8D5}\textbf{1$^{\mathbf{(1)}}$}     & \cellcolor[HTML]{D5E8D5}0.708 & \cellcolor[HTML]{D5E8D5}\textbf{3.427$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.604 & \cellcolor[HTML]{D5E8D5}\textbf{4.8288$^{\mathbf{(1)}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.472} & \cellcolor[HTML]{D5E8D5}\textbf{1.2855$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.49  & \cellcolor[HTML]{D5E8D5}3.437$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.531 & \cellcolor[HTML]{D5E8D5}4.869$^{\mathbf{(3)}}$              & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.485} \\ \hline
\multicolumn{1}{c}{}                                    & \multicolumn{18}{c}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\
\multicolumn{1}{c}{\multirow{-2}{*}{}}                  & \multicolumn{18}{c}{\multirow{-2}{*}{\textbf{Test data: Daegu (GDP)}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \hline
\multicolumn{1}{|c|}{}                                  & \multicolumn{6}{c|}{\textbf{Training data: Daegu}}                                                                                                                                                                                                                                                & \multicolumn{6}{c|}{\textbf{Training data: Seoul}}                                                                                                                                                                                                                                                & \multicolumn{6}{c|}{\textbf{Training data: Taichung}}                                                                                                                                                                                                                                                 \\ \cline{2-19} 
\multicolumn{1}{|c|}{}                                  & \multicolumn{2}{c|}{p=0.1}                                                               & \multicolumn{2}{c|}{p=0.5}                                                              & \multicolumn{2}{c|}{p=0.9}                                                                                   & \multicolumn{2}{c|}{p=0.1}                                                              & \multicolumn{2}{c|}{p=0.5}                                                              & \multicolumn{2}{c|}{p=0.9}                                                                                    & \multicolumn{2}{c|}{p=0.1}                                                               & \multicolumn{2}{c|}{p=0.5}                                                              & \multicolumn{2}{c|}{p=0.9}                                                                                       \\ \cline{2-19} 
\multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Method}}} & \multicolumn{1}{c}{$\mu$}                                & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                                & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                                & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                                   & \multicolumn{1}{c|}{$\sigma$}                      \\ \hline
\multicolumn{1}{|l|}{OK}                                & \cellcolor[HTML]{D5E8D5}2.5744$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.277 & \cellcolor[HTML]{D5E8D5}2.69$^{\mathbf{(3)}}$           & \cellcolor[HTML]{D5E8D5}0.33  & \cellcolor[HTML]{D5E8D5}2.733$^{\mathbf{(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.264} & \cellcolor[HTML]{F8CECC}9.953$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.767 & \cellcolor[HTML]{F8CECC}10.19$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.68  & \cellcolor[HTML]{F8CECC}10.097$^{(\otimes)}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}0.749} & \cellcolor[HTML]{D5E8D5}2.4427$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.268 & \cellcolor[HTML]{D5E8D5}2.572$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.217 & \cellcolor[HTML]{D5E8D5}2.645$^{\mathbf{(2),(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.234} \\
\multicolumn{1}{|l|}{UK}                                & 2.7399                                                   & 0.253                         & \cellcolor[HTML]{D5E8D5}2.652$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.269 & \cellcolor[HTML]{D5E8D5}2.634$^{\mathbf{(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.242} & \cellcolor[HTML]{F8CECC}10.25$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.615 & \cellcolor[HTML]{F8CECC}9.917$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.647 & \cellcolor[HTML]{F8CECC}10.113$^{(\otimes)}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}0.947} & 2.6752                                                   & 0.262                         & 2.635                                                   & 0.308                         & \cellcolor[HTML]{D5E8D5}2.639$^{\mathbf{(2),(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.278} \\
\multicolumn{1}{|l|}{Basic}                             & \cellcolor[HTML]{D5E8D5}0.9115$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}0.054 & \cellcolor[HTML]{D5E8D5}0.87$^{\mathbf{(2)}}$           & \cellcolor[HTML]{D5E8D5}0.174 & \cellcolor[HTML]{D5E8D5}\textbf{0.885$^{\mathbf{(1)}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.738} & 3.563                                                   & 1.457                         & 3.844                                                   & 0.413                         & 3.9103                                                   & \multicolumn{1}{l|}{0.111}                         & 2.9415                                                   & 1.177                         & 3.555                                                   & 0.527                         & 3.497                                                       & \multicolumn{1}{l|}{0.155}                         \\
\multicolumn{1}{|l|}{SAR}                               & 2.3524                                                   & 0.97                          & 2.76                                                    & 21.83                         & 3.13                                                    & \multicolumn{1}{l|}{1.635}                         & 4.657                                                   & 1.606                         & 3.7                                                     & 1.422                         & 3.8877                                                   & \multicolumn{1}{l|}{1.369}                         & 3.1096                                                   & 0.342                         & 3.231                                                   & 1.871                         & 3.087                                                       & \multicolumn{1}{l|}{1.29}                          \\
\multicolumn{1}{|l|}{MA}                                & \cellcolor[HTML]{F8CECC}3.5148$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.476 & \cellcolor[HTML]{F8CECC}3.827$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.659 & \cellcolor[HTML]{F8CECC}4.529$^{(\otimes)}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}12.18} & 4.188                                                   & 2.078                         & 5.653                                                   & 2.404                         & 4.2532                                                   & \multicolumn{1}{l|}{3.829}                         & \cellcolor[HTML]{F8CECC}3.9726$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.575 & \cellcolor[HTML]{F8CECC}3.973$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}4.31  & \cellcolor[HTML]{F8CECC}3.869$^{(\otimes)}$                 & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}27.54} \\
\multicolumn{1}{|l|}{ARMA}                              & \cellcolor[HTML]{F8CECC}3.4663$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}0.985 & \cellcolor[HTML]{F8CECC}4.082$^{(\otimes)}$             & \cellcolor[HTML]{F8CECC}1.065 & \cellcolor[HTML]{F8CECC}3.332$^{(\otimes)}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}5.114} & 4.225                                                   & 1.181                         & 4.957                                                   & 1.326                         & 4.7411                                                   & \multicolumn{1}{l|}{1.559}                         & 3.6237                                                   & 1.151                         & 3.9                                                     & 0.773                         & \cellcolor[HTML]{F8CECC}3.973$^{(\otimes)}$                 & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}0.359} \\
\multicolumn{1}{|l|}{CNN}                               & 3.0502                                                   & 0.201                         & 2.978                                                   & 1.789                         & 3.297                                                   & \multicolumn{1}{l|}{1.206}                         & 3.087                                                   & 0.165                         & \cellcolor[HTML]{D5E8D5}3.088$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.165 & \cellcolor[HTML]{D5E8D5}3.0874$^{\mathbf{(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.164} & 3.08                                                     & 0.17                          & 3.086                                                   & 0.405                         & 3.083                                                       & \multicolumn{1}{l|}{0.152}                         \\ \hline
\multicolumn{1}{|l|}{SD-MRP}                            & 2.0795                                                   & 1.324                         & \cellcolor[HTML]{D5E8D5}2.31$^{\mathbf{(3)}}$           & \cellcolor[HTML]{D5E8D5}0.658 & \cellcolor[HTML]{D5E8D5}2.838$^{\mathbf{(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.346} & \cellcolor[HTML]{D5E8D5}1.814$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}1.202 & \cellcolor[HTML]{D5E8D5}2.028$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}0.347 & \cellcolor[HTML]{D5E8D5}2.8601$^{\mathbf{(2)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.338} & \cellcolor[HTML]{D5E8D5}1.5947$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}1.031 & \cellcolor[HTML]{D5E8D5}2.155$^{\mathbf{(2)}}$          & \cellcolor[HTML]{D5E8D5}0.453 & \cellcolor[HTML]{D5E8D5}2.691$^{\mathbf{(2),(3)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.275} \\
\multicolumn{1}{|l|}{WP-MRP}                            & 2.1978                                                   & 1.359                         & 2.928                                                   & 0.62                          & 2.981                                                   & \multicolumn{1}{l|}{0.218}                         & \cellcolor[HTML]{D5E8D5}2.746$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}1.534 & \cellcolor[HTML]{D5E8D5}3.162$^{\mathbf{(3)}}$          & \cellcolor[HTML]{D5E8D5}0.651 & 3.0168                                                   & \multicolumn{1}{l|}{0.228}                         & 6.0888                                                   & 2.464                         & 5.322                                                   & 0.781                         & 5.205                                                       & \multicolumn{1}{l|}{0.297}                         \\ \hline
\multicolumn{1}{|l|}{O-MRP}                             & \cellcolor[HTML]{D5E8D5}\textbf{0.4538$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.257 & \cellcolor[HTML]{D5E8D5}\textbf{0.78$^{\mathbf{(1)}}$}  & \cellcolor[HTML]{D5E8D5}0.137 & \cellcolor[HTML]{D5E8D5}1.377$^{\mathbf{(2)}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.45}  & \cellcolor[HTML]{D5E8D5}\textbf{0.442$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.327 & \cellcolor[HTML]{D5E8D5}\textbf{1.411$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.252 & \cellcolor[HTML]{D5E8D5}\textbf{2.3357$^{\mathbf{(1)}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.352} & \cellcolor[HTML]{D5E8D5}\textbf{0.4436$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.243 & \cellcolor[HTML]{D5E8D5}\textbf{1.484$^{\mathbf{(1)}}$} & \cellcolor[HTML]{D5E8D5}0.251 & \cellcolor[HTML]{D5E8D5}\textbf{2.448$^{\mathbf{(1)}}$}     & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.328} \\ \hline
\end{tabular}%
}
\caption{Results for GDP interpolation methods in terms of the MAE mean and standard deviation from 30 runs per condition. The errors in this table have been divided by $10^{4}$ for convenient readability. The first to third best performing methods have been marked with the superscript $\mu^{(1)}$, $\mu^{(2)}$ or $\mu^{(3)}$ and a green background, and the worst performing method has been marked with $\mu^{(\otimes)}$ and a red background. Rankings were determined using statistical significance testing at $\alpha=0.05$  (ties allowed). The lowest error per condition, regardless of statistical significance, was marked \textbf{bold}.}
\label{tab:gdp}
\end{table}





% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% % \usepackage[table,xcdraw]{xcolor}
% % If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[]
% \centering
% \resizebox{0.95\textwidth}{!}{%
% \begin{tabular}{lllllllllllllllllll}
% \hline
% \multicolumn{1}{c}{}                                    & \multicolumn{18}{c}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\
% \multicolumn{1}{c}{\multirow{-2}{*}{}}                  & \multicolumn{18}{c}{\multirow{-2}{*}{\textbf{Test data:   Taipei (GDP)}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
% \multicolumn{1}{|c|}{}                                  & \multicolumn{6}{c|}{\textbf{Training data: Taipei}}                                                                                                                                                                                                                                         & \multicolumn{6}{c|}{\textbf{Training data: Seoul}}                                                                                                                                                                                                                                          & \multicolumn{6}{c|}{\textbf{Training data: Taichung}}                                                                                                                                                                                                                                         \\ \cline{2-19} 
% \multicolumn{1}{|c|}{}                                  & \multicolumn{2}{c|}{p=0.1}                                                             & \multicolumn{2}{c|}{p=0.5}                                                            & \multicolumn{2}{c|}{p=0.9}                                                                                 & \multicolumn{2}{c|}{p=0.1}                                                            & \multicolumn{2}{c|}{p=0.5}                                                            & \multicolumn{2}{c|}{p=0.9}                                                                                  & \multicolumn{2}{c|}{p=0.1}                                                             & \multicolumn{2}{c|}{p=0.5}                                                            & \multicolumn{2}{c|}{p=0.9}                                                                                   \\ \cline{2-19} 
% \multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Method}}} & \multicolumn{1}{c}{$\mu$}                              & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                              & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                              & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$}                      \\ \hline
% \multicolumn{1}{|l|}{OK}                                & \cellcolor[HTML]{D5E8D5}2.6301$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.233 & \cellcolor[HTML]{D5E8D5}2.629$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.244 & \cellcolor[HTML]{D5E8D5}\textbf{2.615$^{\mathbf{1}}$} & \multicolumn{1}{l|}{0.232}                         & 10.11                                                 & 0.589                         & 10.15                                                 & 0.583                         & 9.8365                                                 & \multicolumn{1}{l|}{0.465}                         & \cellcolor[HTML]{D5E8D5}2.5661$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.276 & \cellcolor[HTML]{D5E8D5}\textbf{2.504$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.233 & \cellcolor[HTML]{D5E8D5}2.692$^{\mathbf{1,2}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.252} \\
% \multicolumn{1}{|l|}{UK}                                & \cellcolor[HTML]{D5E8D5}2.6704$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.236 & \cellcolor[HTML]{D5E8D5}2.593$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.223 & \cellcolor[HTML]{D5E8D5}2.727$^{\mathbf{2}}$          & \multicolumn{1}{l|}{0.249}                         & 10.19                                                 & 0.835                         & 10.41                                                 & 0.659                         & 10.317                                                 & \multicolumn{1}{l|}{0.74}                          & \cellcolor[HTML]{D5E8D5}2.6261$^{\mathbf{2,3}}$        & \cellcolor[HTML]{D5E8D5}0.24  & \cellcolor[HTML]{D5E8D5}2.601$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}0.382 & \cellcolor[HTML]{D5E8D5}\textbf{2.649$^{\mathbf{1,2}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.223} \\
% \multicolumn{1}{|l|}{Basic}                             & 3.9129                                                 & 0.108                         & 3.779                                                 & 0.355                         & 3.451                                                 & \multicolumn{1}{l|}{0.857}                         & \cellcolor[HTML]{F8CECC}26.68$^{\otimes}$             & \cellcolor[HTML]{F8CECC}4.757 & \cellcolor[HTML]{F8CECC}26.27$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.704 & \cellcolor[HTML]{F8CECC}26.483$^{\otimes}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}0.306} & 4.9292                                                 & 1.705                         & 5.225                                                 & 0.753                         & 5.069                                                   & \multicolumn{1}{l|}{0.24}                          \\
% \multicolumn{1}{|l|}{SAR}                               & 3.5778                                                 & 0.532                         & 4.164                                                 & 0.488                         & \cellcolor[HTML]{F8CECC}5.709$^{\otimes}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}1.659} & 7.972                                                 & 1037                          & 8.681                                                 & 1.585                         & 8.6299                                                 & \multicolumn{1}{l|}{1.298}                         & 5.7945                                                 & 2.396                         & \cellcolor[HTML]{F8CECC}5.913$^{\otimes}$             & \cellcolor[HTML]{F8CECC}13.95 & \cellcolor[HTML]{F8CECC}6.018$^{\otimes}$               & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}104.5} \\
% \multicolumn{1}{|l|}{MA}                                & 3.664                                                  & 0.556                         & 3.745                                                 & 0.505                         & 4.204                                                 & \multicolumn{1}{l|}{1.827}                         & 9.064                                                 & 8.498                         & 8.413                                                 & 5.201                         & 9.0289                                                 & \multicolumn{1}{l|}{12.25}                         & \cellcolor[HTML]{F8CECC}6.4553$^{\otimes}$             & \cellcolor[HTML]{F8CECC}2277  & \cellcolor[HTML]{F8CECC}6.365$^{\otimes}$             & \cellcolor[HTML]{F8CECC}22.67 & 6.083                                                   & \multicolumn{1}{l|}{17.24}                         \\
% \multicolumn{1}{|l|}{ARMA}                              & 3.9379                                                 & 0.569                         & 4.067                                                 & 0.728                         & 4.386                                                 & \multicolumn{1}{l|}{0.689}                         & 9.46                                                  & 5.503                         & 9.446                                                 & 7.303                         & 10.939                                                 & \multicolumn{1}{l|}{4.77}                          & 5.4766                                                 & 0.884                         & 5.443                                                 & 1.067                         & 6.15                                                    & \multicolumn{1}{l|}{1.072}                         \\
% \multicolumn{1}{|l|}{CNN}                               & \cellcolor[HTML]{F8CECC}5.469$^{\otimes}$              & \cellcolor[HTML]{F8CECC}0.378 & \cellcolor[HTML]{F8CECC}5.481$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.811 & 4.79                                                  & \multicolumn{1}{l|}{2.259}                         & \cellcolor[HTML]{D5E8D5}5.676$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.242 & 5.606                                                 & 0.245                         & \cellcolor[HTML]{D5E8D5}5.7203$^{\mathbf{3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.238} & 5.5233                                                 & 2.251                         & 5.509                                                 & 1.454                         & 5.537                                                   & \multicolumn{1}{l|}{13.89}                         \\ \hline
% \multicolumn{1}{|l|}{SD-MRP}                            & 3.7774                                                 & 1.981                         & 4.585                                                 & 0.736                         & 5.262                                                 & \multicolumn{1}{l|}{0.329}                         & \cellcolor[HTML]{D5E8D5}3.695$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}1.348 & \cellcolor[HTML]{D5E8D5}4.582$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}0.508 & \cellcolor[HTML]{D5E8D5}5.3042$^{\mathbf{2}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.557} & 3.869                                                  & 1.451                         & 4.301                                                 & 0.409                         & \cellcolor[HTML]{D5E8D5}4.75$^{\mathbf{3}}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.442} \\
% \multicolumn{1}{|l|}{WP-MRP}                            & 4.9688                                                 & 2.243                         & \cellcolor[HTML]{F8CECC}5.382$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.723 & 5.296                                                 & \multicolumn{1}{l|}{0.263}                         & \cellcolor[HTML]{D5E8D5}6.089$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}2.464 & \cellcolor[HTML]{D5E8D5}5.322$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.781 & 5.2046                                                 & \multicolumn{1}{l|}{0.297}                         & 5.4675                                                 & 2.538                         & 5.284                                                 & 0.962                         & 5.183                                                   & \multicolumn{1}{l|}{0.319}                         \\ \hline
% \multicolumn{1}{|l|}{O-MRP}                             & \cellcolor[HTML]{D5E8D5}\textbf{0.9534$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.514 & \cellcolor[HTML]{D5E8D5}\textbf{1.753$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.343 & \cellcolor[HTML]{D5E8D5}3.021$^{\mathbf{3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.746} & \cellcolor[HTML]{D5E8D5}\textbf{1$^{\mathbf{1}}$}     & \cellcolor[HTML]{D5E8D5}0.708 & \cellcolor[HTML]{D5E8D5}\textbf{3.427$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.604 & \cellcolor[HTML]{D5E8D5}\textbf{4.8288$^{\mathbf{1}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.472} & \cellcolor[HTML]{D5E8D5}\textbf{1.2855$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.49  & \cellcolor[HTML]{D5E8D5}3.437$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.531 & \cellcolor[HTML]{D5E8D5}4.869$^{\mathbf{3}}$            & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.485} \\ \hline
% \multicolumn{1}{c}{}                                    & \multicolumn{18}{c}{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\
% \multicolumn{1}{c}{\multirow{-2}{*}{}}                  & \multicolumn{18}{c}{\multirow{-2}{*}{\textbf{Test data: Daegu (GDP)}}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
% \multicolumn{1}{|c|}{}                                  & \multicolumn{6}{c|}{\textbf{Training data: Daegu}}                                                                                                                                                                                                                                          & \multicolumn{6}{c|}{\textbf{Training data: Seoul}}                                                                                                                                                                                                                                          & \multicolumn{6}{c|}{\textbf{Training data: Taichung}}                                                                                                                                                                                                                                         \\ \cline{2-19} 
% \multicolumn{1}{|c|}{}                                  & \multicolumn{2}{c|}{p=0.1}                                                             & \multicolumn{2}{c|}{p=0.5}                                                            & \multicolumn{2}{c|}{p=0.9}                                                                                 & \multicolumn{2}{c|}{p=0.1}                                                            & \multicolumn{2}{c|}{p=0.5}                                                            & \multicolumn{2}{c|}{p=0.9}                                                                                  & \multicolumn{2}{c|}{p=0.1}                                                             & \multicolumn{2}{c|}{p=0.5}                                                            & \multicolumn{2}{c|}{p=0.9}                                                                                   \\ \cline{2-19} 
% \multicolumn{1}{|c|}{\multirow{-3}{*}{\textbf{Method}}} & \multicolumn{1}{c}{$\mu$}                              & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                              & \multicolumn{1}{c|}{$\sigma$}                      & \multicolumn{1}{c}{$\mu$}                              & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                             & \multicolumn{1}{c|}{$\sigma$} & \multicolumn{1}{c}{$\mu$}                               & \multicolumn{1}{c|}{$\sigma$}                      \\ \hline
% \multicolumn{1}{|l|}{OK}                                & \cellcolor[HTML]{D5E8D5}2.5744$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.277 & \cellcolor[HTML]{D5E8D5}2.69$^{\mathbf{3}}$           & \cellcolor[HTML]{D5E8D5}0.33  & \cellcolor[HTML]{D5E8D5}2.733$^{\mathbf{3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.264} & \cellcolor[HTML]{F8CECC}9.953$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.767 & \cellcolor[HTML]{F8CECC}10.19$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.68  & \cellcolor[HTML]{F8CECC}10.097$^{\otimes}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}0.749} & \cellcolor[HTML]{D5E8D5}2.4427$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.268 & \cellcolor[HTML]{D5E8D5}2.572$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.217 & \cellcolor[HTML]{D5E8D5}2.645$^{\mathbf{2,3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.234} \\
% \multicolumn{1}{|l|}{UK}                                & 2.7399                                                 & 0.253                         & \cellcolor[HTML]{D5E8D5}2.652$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.269 & \cellcolor[HTML]{D5E8D5}2.634$^{\mathbf{3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.242} & \cellcolor[HTML]{F8CECC}10.25$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.615 & \cellcolor[HTML]{F8CECC}9.917$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.647 & \cellcolor[HTML]{F8CECC}10.113$^{\otimes}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}0.947} & 2.6752                                                 & 0.262                         & 2.635                                                 & 0.308                         & \cellcolor[HTML]{D5E8D5}2.639$^{\mathbf{2,3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.278} \\
% \multicolumn{1}{|l|}{Basic}                             & \cellcolor[HTML]{D5E8D5}0.9115$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}0.054 & \cellcolor[HTML]{D5E8D5}0.87$^{\mathbf{2}}$           & \cellcolor[HTML]{D5E8D5}0.174 & \cellcolor[HTML]{D5E8D5}\textbf{0.885$^{\mathbf{1}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.738} & 3.563                                                 & 1.457                         & 3.844                                                 & 0.413                         & 3.9103                                                 & \multicolumn{1}{l|}{0.111}                         & 2.9415                                                 & 1.177                         & 3.555                                                 & 0.527                         & 3.497                                                   & \multicolumn{1}{l|}{0.155}                         \\
% \multicolumn{1}{|l|}{SAR}                               & 2.3524                                                 & 0.97                          & 2.76                                                  & 21.83                         & 3.13                                                  & \multicolumn{1}{l|}{1.635}                         & 4.657                                                 & 1.606                         & 3.7                                                   & 1.422                         & 3.8877                                                 & \multicolumn{1}{l|}{1.369}                         & 3.1096                                                 & 0.342                         & 3.231                                                 & 1.871                         & 3.087                                                   & \multicolumn{1}{l|}{1.29}                          \\
% \multicolumn{1}{|l|}{MA}                                & \cellcolor[HTML]{F8CECC}3.5148$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.476 & \cellcolor[HTML]{F8CECC}3.827$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.659 & \cellcolor[HTML]{F8CECC}4.529$^{\otimes}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}12.18} & 4.188                                                 & 2.078                         & 5.653                                                 & 2.404                         & 4.2532                                                 & \multicolumn{1}{l|}{3.829}                         & \cellcolor[HTML]{F8CECC}3.9726$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.575 & \cellcolor[HTML]{F8CECC}3.973$^{\otimes}$             & \cellcolor[HTML]{F8CECC}4.31  & \cellcolor[HTML]{F8CECC}3.869$^{\otimes}$               & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}27.54} \\
% \multicolumn{1}{|l|}{ARMA}                              & \cellcolor[HTML]{F8CECC}3.4663$^{\otimes}$             & \cellcolor[HTML]{F8CECC}0.985 & \cellcolor[HTML]{F8CECC}4.082$^{\otimes}$             & \cellcolor[HTML]{F8CECC}1.065 & \cellcolor[HTML]{F8CECC}3.332$^{\otimes}$             & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}5.114} & 4.225                                                 & 1.181                         & 4.957                                                 & 1.326                         & 4.7411                                                 & \multicolumn{1}{l|}{1.559}                         & 3.6237                                                 & 1.151                         & 3.9                                                   & 0.773                         & \cellcolor[HTML]{F8CECC}3.973$^{\otimes}$               & \multicolumn{1}{l|}{\cellcolor[HTML]{F8CECC}0.359} \\
% \multicolumn{1}{|l|}{CNN}                               & 3.0502                                                 & 0.201                         & 2.978                                                 & 1.789                         & 3.297                                                 & \multicolumn{1}{l|}{1.206}                         & 3.087                                                 & 0.165                         & \cellcolor[HTML]{D5E8D5}3.088$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.165 & \cellcolor[HTML]{D5E8D5}3.0874$^{\mathbf{3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.164} & 3.08                                                   & 0.17                          & 3.086                                                 & 0.405                         & 3.083                                                   & \multicolumn{1}{l|}{0.152}                         \\ \hline
% \multicolumn{1}{|l|}{SD-MRP}                            & 2.0795                                                 & 1.324                         & \cellcolor[HTML]{D5E8D5}2.31$^{\mathbf{3}}$           & \cellcolor[HTML]{D5E8D5}0.658 & \cellcolor[HTML]{D5E8D5}2.838$^{\mathbf{3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.346} & \cellcolor[HTML]{D5E8D5}1.814$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}1.202 & \cellcolor[HTML]{D5E8D5}2.028$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}0.347 & \cellcolor[HTML]{D5E8D5}2.8601$^{\mathbf{2}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.338} & \cellcolor[HTML]{D5E8D5}1.5947$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}1.031 & \cellcolor[HTML]{D5E8D5}2.155$^{\mathbf{2}}$          & \cellcolor[HTML]{D5E8D5}0.453 & \cellcolor[HTML]{D5E8D5}2.691$^{\mathbf{2,3}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.275} \\
% \multicolumn{1}{|l|}{WP-MRP}                            & 2.1978                                                 & 1.359                         & 2.928                                                 & 0.62                          & 2.981                                                 & \multicolumn{1}{l|}{0.218}                         & \cellcolor[HTML]{D5E8D5}2.746$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}1.534 & \cellcolor[HTML]{D5E8D5}3.162$^{\mathbf{3}}$          & \cellcolor[HTML]{D5E8D5}0.651 & 3.0168                                                 & \multicolumn{1}{l|}{0.228}                         & 6.0888                                                 & 2.464                         & 5.322                                                 & 0.781                         & 5.205                                                   & \multicolumn{1}{l|}{0.297}                         \\ \hline
% \multicolumn{1}{|l|}{O-MRP}                             & \cellcolor[HTML]{D5E8D5}\textbf{0.4538$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.257 & \cellcolor[HTML]{D5E8D5}\textbf{0.78$^{\mathbf{1}}$}  & \cellcolor[HTML]{D5E8D5}0.137 & \cellcolor[HTML]{D5E8D5}1.377$^{\mathbf{2}}$          & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.45}  & \cellcolor[HTML]{D5E8D5}\textbf{0.442$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.327 & \cellcolor[HTML]{D5E8D5}\textbf{1.411$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.252 & \cellcolor[HTML]{D5E8D5}\textbf{2.3357$^{\mathbf{1}}$} & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.352} & \cellcolor[HTML]{D5E8D5}\textbf{0.4436$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.243 & \cellcolor[HTML]{D5E8D5}\textbf{1.484$^{\mathbf{1}}$} & \cellcolor[HTML]{D5E8D5}0.251 & \cellcolor[HTML]{D5E8D5}\textbf{2.448$^{\mathbf{1}}$}   & \multicolumn{1}{l|}{\cellcolor[HTML]{D5E8D5}0.328} \\ \hline
% \end{tabular}%
% }
% \caption{Results for GDP interpolation methods in terms of the MAE mean and standard deviation from 30 runs per condition. The errors in this table have been divided by $10^{4}$ for convenient readability. The first to third best performing methods have been marked with the superscript $\mu^{1}$, $\mu^{2}$ or $\mu^{3}$ and a green background, and the worst performing method has been marked with $\mu^{\otimes}$ and a red background. Rankings were determined using statistical significance testing at $\alpha=0.05$  (ties allowed). The lowest error per condition, regardless of statistical significance, was marked \textbf{bold}.}
% \label{tab:gdp}
% \end{table*}







==> Chapters/related_work.tex <==
To date, various spatial interpolation methods have been proposed. 
%\mb{for spatial interpolation have been proposed}
For convenience, we will categorise methods into (i) \textit{purely spatial methods}, and (ii) \textit{spatial methods with explanatory variables}. Purely spatial methods consist of those models relying solely on known true values and their spatial locations to fill in the grid: $\hat{y}_{c} := \mathcal{M}(\mathbf{Y})$. Conversely, spatial methods with explanatory variables predict $\hat{y}_{c}$ using explanatory variables: $\hat{y}_{c} := \mathcal{M}(\mathbf{Y},\mathbf{x}_{c})$.

\section{Purely spatial methods}
Given the widespread use of kriging-based interpolation, we will sub-categorise the purely spatial methods further into kriging and non-kriging methods.
\subsection{Kriging}
Kriging, also known as Gaussian processes, is an interpolation technique based on learning the covariance of target values over distance using variogram (kernel) functions fitted to the data. Popular variants of kriging include ordinary kriging (OK), universal kriging (UK), regression kriging (kriging after detrending) and kriging with external drift \cite{jiang2018survey}. 
The difference between kriging variants tends to lie in the degree to which they assume stationarity and isotropy. Contemporary contributions to the kriging field include a scalable gradient-based surrogate function method \cite{bouhlel2019gradient} and a neural network-based method to overcome kriging's limitation of disregarding the characteristics of intermediate locations in paths between pairs of locations \cite{sato2019performance}. \\
Regardless of the degree to which stationarity and isotropy is assumed by any variant, all kriging-based methods are limited by their reliance on pair-wise distance-based covariance models. Intermediate locations are not considered, and explanatory features are typically only used to compensate for trends in the data. However, depending on the region and dataset in question, kriging can perform very well,  %\laurens{Needs references}, 
and can be applied fairly easily to any grid.
\subsection{Non-kriging methods}
In addition to kriging, we will describe four non-kriging methods frequently applied to spatial interpolation. 
%\mb{weird sentence, have commonly used?}. 
First, there is \textbf{inverse distance weighting} \cite{shepard1968two} (IDW), with recent contributions including a new probabilistic weighting scheme \cite{lukaszyk2004new} and an adaptive weighting approach \cite{lu2008adaptive}. Second, a simple \textbf{nearest neighbour} (NN) algorithm could be used for spatial interpolation \cite{olivier2012nearest} \cite{song2017efficient}. Third, a more sophisticated alternative to NN would be the Voronoi polygon-based \cite{voronoi1908nouvelles} \textbf{natural neighbour} algorithm, also known as Sibson interpolation  \cite{sibson1981brief}, for which recent work has often focused on improvements to the efficiency of the algorithm \cite{ledoux2005efficient} \cite{park2006discrete}. Finally, we consider \textbf{spline} interpolation \cite{harder1972interpolation}, where much recent work has also been focused on finding efficient solutions for large-scale datasets \cite{hancock2006spatial}, although it is also seeing applications in problems such as  
%\mb{in problems such as} 
remote sensing data downscaling \cite{sharifi2019downscaling}.\\
As in the case of kriging, methods like IDW and spline interpolation rely heavily on distance-based interactions between points, and do not account for the characteristics of intermediate locations. Conversely, nearest neighbour and natural neighbour interpolation only consider %\mb{ strictly defined neighbours? or pre-defined neighborhoods} 
locations within a pre-defined neighbourhood, and thus do not allow for spatial interaction beyond a certain threshold. 

\section{Spatial methods with explanatory variables}
In this category, 
%\mb{,} 
we will cover four regression models explicitly modelling the spatial properties of the data while also allowing the use of explanatory variables, as well as deep learning models. \\
%\mb{models, approaches}.\\
First, \textbf{spatial autoregressive} models \cite{anselin1988spatial} (SAR) have remained relatively consistent, but have been expanded in some recent work \cite{yang2017identification} \cite{fix2020simultaneous}. \textbf{Moving average} (MA) models are often used in the context of time-series modelling \cite{durbin1959efficient}, 
%\mb{modelling} 
but can also be used for spatial regression problems using the ``MA by AR'' approach \cite{haining1978moving}. Highly related to SAR and MA models, \textbf{autoregressive moving average} (ARMA) models have 
%\mb{have} 
seen a recent early-access paper of particular relevance to the current COVID-19
%\mb{COVID-19} 
pandemic, modelling a transmission network of influenza \cite{qiu2020spatial}. 
%\laurens{I kind of feel like removing GWR since I don't have that much to say about it, but "all relevant citations" must be present...}
\textbf{Geographically weighted regression} (GWR) explicitly assumes non-stationarity and uses the geographic location of the cell to select spatial weights \cite{fotheringham1998geographically}.\\
Finally, deep learning and \textbf{convolutional neural networks} (CNN) in particular have been used to great effect in many computer vision applications \cite{dong2015image} \cite{shi2016real}. These computer vision-based interpolation CNNs could also be applied to general spatial interpolation. Moreover, in their 2020 publication, Hashimoto and Suto formulated a CNN architecture for the specific purpose of spatial interpolation \cite{hashimoto2020sicnn}. \\
As in the case of nearest neighbour and natural neighbour interpolation, this category of methods is limited by their use of a pre-defined local neighbourhood, dismissing information outside of the neighbourhood radius. 
%\mb{the neighbourhood radius}.
%\mb{What is the downside of these works? What is the difference of this paper and the works in the category?}
